VLIPP: Towards Physically Plausible Video Generation with Vision and Language Informed Physical Prior

Video diffusion models (VDMs) have advanced significantly in recent years, enabling the generation of highly realistic videos and drawing the attention of the community in their potential as world simulators. However, despite their capabilities, VDMs often fail to produce physically plausible videos due to an inherent lack of understanding of physics, resulting in incorrect dynamics and event sequences. To address this limitation, we propose a novel two-stage image-to-video generation framework that explicitly incorporates physics with vision and language informed physical prior. In the first stage, we employ a Vision Language Model (VLM) as a coarse-grained motion planner, integrating chain-of-thought and physics-aware reasoning to predict a rough motion trajectories/changes that approximate real-world physical dynamics while ensuring the inter-frame consistency. In the second stage, we use the predicted motion trajectories/changes to guide the video generation of a VDM. As the predicted motion trajectories/changes are rough, noise is added during inference to provide freedom to the VDM in generating motion with more fine details. Extensive experimental results demonstrate that our framework can produce physically plausible motion, and comparative evaluations highlight the notable superiority of our approach over existing methods. More video results are available on our Project Page: https://madaoer.github.io/projects/physically_plausible_video_generation.

==> sec_arxiv/2_Background_Old.tex <==
\section{Related Work}
\label{sec:background}

\subsection{Physically Plausible Video Generation and Challenges
}

Generating physically plausible videos offers substantial value to real-world applications such as scientific simulations\cite{sun2024bora}, robotics~\cite{yang2023learning, bar2024navigation}, and autonomous driving~\cite{wang2024drivedreamer, deng2024streetscapes}. Traditional graphic pipelines rely on physical simulation systems for modeling~\cite{nealen2006physically, stomakhin2013material}. However, these rule-based or solver-based simulators face limitations in expressiveness, efficiency, generalizability, and parameter tuning. Furthermore, these simulators require significant expertise, rendering them inaccessible and unfriendly for users.

Recently, DiT-based VDMs have demonstrated potential in generating videos with both visual and physical realism, even enabling the synthesis tasks that are challenging from a simulation perspective~\cite{yang2024cogvideox, polyak2025moviegencastmedia, jin2024pyramidal, zheng2024open, li2024hunyuan, li2024generative}. Despite their high visual fidelity, the videos generated by DiT-based VDMs do not consistently adhere to physical laws~\cite{meng2024towards, bansal2024videophy, motamed2025generative}. Existing diffusion models are primarily controlled by text and image inputs. However, as shown in Figure~\ref{fig:onecol}, even with detailed textual description of the physical process, the VDMs fail to generate videos that accurately follow the physical laws. This limitation stems from the inability of VDMs in understanding physical laws. 

Several other studies focus on motion-controllable VDMs, mainly offering three forms of user-guided controls: bounding box control~\cite{huang2023fine, li2023trackdiffusion, ma2024trailblazer, wang2024boximator, wu2024motionbooth}, point trajectory control~\cite{mou2024revideo, niu2024mofa, qiu2024freetraj, wang2024motionctrl, wu2024draganything} and camera control~\cite{bahmani2024ac3d, he2024cameractrl, wang2024akira, yu2024viewcrafter}. However, these approaches prioritize motion control but often overlook physical plausibility. To address the limitation, we propose a novel framework for physically plausible video generation that incorporates physics as conditions for video diffusion models.

\begin{figure*}[t]
  \centering
    \includegraphics[width=1.0\linewidth]{Arxiv_tex/Figures/Illustrative_Figure/fig2.pdf}
    \caption{The illustration of our physically plausible image-to-video generation pipeline. Our pipeline consists of two stages. In the first stage, the VLM generates a coarse-grained, physically plausible motion trajectory based on the provided input conditions. In the second stage, We simulate a synthetic video using the predicted trajectory to provide the motion condition. We then extract the optical flow from this video and convert it into structured noise. These conditions are fed into a motion controllable image-to-video diffusion model, and ultimately generates a physically plausible video.}
  \label{fig:2}
  \vspace{-12pt}
\end{figure*}



\subsection{VLM Planning}

VLMs have exhibited robust capabilities in visual understanding and planning. Their strong performance in domains such as robot path planning and video understanding shows their ability in understanding the real physical world.

Prior work has successfully leveraged VLMs to guide the layout of images or videos, yielding promising results~\cite{lian2023llm, wu2024self, lin2023videodirectorgpt}. However, these efforts have yet to address interactions with real-world physical phenomena, such as collision, fall, or melting. 

And the absence of visual information can cause severe hallucination issues in language models for spatial planning tasks, leading to problems like overlapping object boundaries, disproportionate scaling, and incorrect planning.
In this paper, we propose utilizing VLMs as coarse-level motion planners within the image space. To enhance the physics understanding of VLMs, we incorporate physics-aware reasoning and Chain of Thought (CoT)~\cite{wei2022chain} into the inference process. Notably, during the VLM planning stage, generating entire physically plausible motion trajectories is not required. Instead, we leverage the generative priors of VDM to produce fine-level physically plausible videos based on coarse-level motion trajectories provided by the VLM.


\subsection{Evaluating Physics in Videos}

Although recent studies have emerged to evaluate the physical reasonableness of video generation models, the evaluation protocol of physical plausibility in videos remains underexplored. PhyGenBench~\cite{meng2024towards} introduced 160 carefully designed prompts related to six physical forms to assess physical plausibility in videos. It employs VLMs to evaluate semantic alignment and physical commonsense alignment. Similarly, Videophy~\cite{bansal2024videophy} utilizes carefully crafted prompts incorporating physical laws and relies on semantic and physics-informed VLMs for evaluation. Moreover, Physical-IQ~\cite{motamed2025generative} contains 66 real-world physical scenarios and measures physical plausibility by comparing generated videos against ground truth. In our experiments, we adopt Physical-IQ and PhysGenBench as benchmarks to assess the physical plausibility of our generated videos.




\begin{figure*}[t]
  \centering
    \includegraphics[width=0.75\linewidth]{Figures/Illustrative_Figure/fig3.pdf}
    % \caption{The illustration of chain-of-thought reasoning in VLM for generating coarse-grained, determine the applicable physical laws for the given scene firstly, the VLM then performs step-by-step reasoning to predict object motions in image space, leveraging physical context and chain-of-thought prompting. The predicted bounding boxes evolve over time according to real-world physics.}
    \caption{The illustration of chain-of-thought reasoning in the VLM for generating a coarse-grained motion trajectory. First off, the VLM determines the corresponding physical laws and its context for the given scene. Then, the VLM performs step-by-step reasoning to predict the physically plausible motions of objects in image space, leveraging physical context and chain-of-thought prompting. Finally, the VLM predicts bounding boxes according to real-world physics.}
  \label{fig:3}
  \vspace{-8pt}
\end{figure*}
z
